Towards Data-Efficient Detection Transformers

Detection Transformers have achieved competitive performance on the sample-rich COCO dataset. However, we show most of them suffer from significant performance drops on small-size datasets, like Cityscapes. In other words, the detection transformers are generally data-hungry. To tackle this problem, we empirically analyze the factors that affect data efficiency, through a step-by-step transition from a data-efficient RCNN variant to the representative DETR. The empirical results suggest that sparse feature sampling from local image areas holds the key. Based on this observation, we alleviate the data-hungry issue of existing detection transformers by simply alternating how key and value sequences are constructed in the cross-attention layer, with minimum modifications to the original models. Besides, we introduce a simple yet effective label augmentation method to provide richer supervision and improve data efficiency. Experiments show that our method can be readily applied to different detection transformers and improve their performance on both small-size and sample-rich datasets. Code will be made publicly available at \url{https://github.com/encounter1997/DE-DETRs}.

==> app_tables/ablate_recipe.tex <==
\begin{table*}[t]
\begin{center}
\setlength{\tabcolsep}{0.12cm}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c}
\Xhline{2\arrayrulewidth}
\hline
\rowcolor{mygray}
{Model} & {Modification} & {50E AP} & {300E AP} & \tabincell{c}{Params} & \tabincell{c}{FLOPs} \\
\hline
SRCN & -- & 29.4 & 35.9 & 106M & 631G \\
\hline
% 300 -> 100
% detrlr, gradnorm
% focal -> ce loss
& change query number & 28.1 (\textcolor{red}{-1.3}) & 33.4 (\textcolor{red}{-2.5}) & 106M & 294G \\
& update learning rate and grad norm & 32.2 (\textcolor{blue}{+4.1}) & 34.6 (\textcolor{blue}{+1.2}) & 106M & 294G \\
\hline
Net1 & change classification loss type & 30.6 (\textcolor{red}{-1.6}) & 34.4 (\textcolor{red}{-0.2}) & 106M & 294G \\
\Xhline{2\arrayrulewidth}
\hline
\end{tabular}
}
\end{center}
\caption{Ablations on DETR and Sparse RCNN (SRCN for short) recipes, experimented on Ciytscapes~\cite{cityscapes}. ``50E AP" and ``300E AP" indicate average precision after training for 50 and 300 epochs, respectively. 
The change in AP is shown in the brackets, where \textcolor{red}{red} indicates drops and \textcolor{blue}{blue} indicates gains on AP.
% Recipe includes classification loss (loss type, relative weight), learning rate (base, lrbackbone), gradnorm, and number of object queries. We use 50e and 300e schedules for a fair comparison. 
}
\label{table: app_ablate_recipe}
\end{table*}

==> app_tables/faster_rcnn.tex <==


\begin{table}[ht]
\renewcommand{\arraystretch}{1.0}
\renewcommand{\tabcolsep}{3.pt}
\centering
\caption{Faster RCNN trained on Cityscapes. $+$ indicates the model is trained with DETR-like data augmentations.}
\label{table: app_compare_city}
    \begin{tabular}{l|c|cccccc|cc}
    \Xhline{2\arrayrulewidth}  
    \hline
    \rowcolor{mygray}
    Method & Epochs & AP & AP$_\text{50}$ & AP$_\text{75}$ & AP$_\text{S}$ & AP$_\text{M}$ & AP$_\text{L}$ & \tabincell{c}{Params} & \tabincell{c}{FLOPs} \\
    % Method & Epochs & AP & AP50 & AP75 & APS & APM & APL & Params & FLOPs & FPS \\
    \hline
    FasterRCNN-FPN & 36 & 32.3 & 56.6 & 31.7 & 10.2 & 32.1 & 53.4 & 41M & 182G \\
    FasterRCNN-FPN$+$ & 36 & 37.3 & 62.5 & 37.3 & 14.0 & 37.6 & 58.2 & 41M & 182G \\
    % 
    \Xhline{2\arrayrulewidth}
    \end{tabular}
\end{table}
